Towards a formally verified implementation of the MimbleWimble cryptocurrency protocol

MimbleWimble is a privacy-oriented cryptocurrency technology encompassing security and scalability properties that distinguish it from other protocols of the kind. In this paper we present and briefly discuss those properties and outline the basis of a model-driven verification approach to address the certification of the correctness of a particular implementation of the protocol.

==> codeverif.tex <==
\section{Source code verification}
\label{sec:source-verification}

%Verification of the correctness of the source code is the ultimate goal of the entire verification process. In this context a working implementation already exits. Then, as a first step towards this goal, a formal specification of the code must be written (see \ref{afsv}). Once that specification has been written it has to be verified...

Verification of the correctness of the source code is the ultimate goal of the entire verification process. We shall take as reference implementation the code available at Grin's GitHub repository.

In what follows we shall illustrate, by means of a simple example, the verification process we have in mind.
%example of the verification process that should be followed. 
For that we consider the Rust code shown in Figure \ref{partialeq} which corresponds to function \verb+PartialEq+ located in \verb+grin/core/src/core/transaction.rs+ of the mentioned repository.
%Grin's GitHub repository. 

This example is not intended to produce 
%by no means 
a final specification of \verb+PartialEq+; in particular, the specification shown below does not necessarily corresponds to a correct semantics of a Rust program. The idea is to give an approximation of the technique that should be used. In particular, the semantics model is a little bit more abstract than it should be. % but this allows to describe the example within this paper.

\begin{figure*}
\footnotesize
%\hly{MEJOR USAR LISTING}
\begin{verbatim}
/// A transaction
#[derive(Serialize, Deserialize, Debug, Clone)]
pub struct Transaction {
    /// List of inputs spent by the transaction.
    pub inputs: Vec<Input>,
    /// List of outputs the transaction produces.
    pub outputs: Vec<Output>,
    /// List of kernels that make up this transaction (usually a single kernel).
    pub kernels: Vec<TxKernel>,
    /// The kernel "offset" k2
    /// excess is k1G after splitting the key k = k1 + k2
    pub offset: BlindingFactor,
}

/// PartialEq
impl PartialEq for Transaction {
    fn eq(&self, tx: &Transaction) -> bool {
        self.inputs     == tx.inputs
        && self.outputs == tx.outputs
        && self.kernels == tx.kernels
        && self.offset  == tx.offset
    }
}
\end{verbatim}
\normalsize
\caption{\label{partialeq}MimbleWinble code snipet (\texttt{PartialEq::grin/core/src/core/transaction.rs})}
\end{figure*}


\subsection{From code to specification}
%The specification of the code is actually its translation into a formal model of Rust's semantics. Therefore, we first need such formal model. There are essentially two ways of getting this model: a) existing models can be taken (and, if necessary, extended or adapted) \cite{DBLP:journals/corr/abs-1804-07608,Reed2015PatinaA} \hly{ojo que parece que ninguno de los dos papers esta publicado; son los unicos dos que encontre en una busqueda ultra rapida}; b) a new model can be written. The main advantage of the first option is the effort savings (although you need to understand it) while its greatest disadvantage is that it might introduce a bias towards a particular verification environment/framework that you would not like to use. In turn the main advantage of the second choice is that you can use the tools that best suits your needs, but it has the disadvantage of taking longer to be ready. 

In this section we will derive a formal specification (of part) of the implementation code. This specification coincides with the specification named $S_2$ in Section \ref{r2sc2s}.

The first step in the process of deriving a formal specification of a portion of code is the choice of the mathematical setting in which shall be expressed the (abstract) semantics of the code. In the case of the Rust code we are presenting as the example one obvious first choice is to adopt, and possibly extend, an already existing formulation of the semantics of that programming language (see \cite{DBLP:journals/corr/abs-1804-07608,Reed2015PatinaA}). 
 An alternative approach would be to write down from scratch the model using the  mathematical and tool setting that better suit the skills of the specification team. Clearly, both approaches have the corresponding pros and cons.

%The specification of the code is actually its translation into a formal model of Rust's semantics. Therefore, we first need such formal model. There are essentially two ways of getting this model: a) existing models can be taken (and, if necessary, extended or adapted) \cite{DBLP:journals/corr/abs-1804-07608,Reed2015PatinaA} \hly{ojo que parece que ninguno de los dos papers esta publicado; son los unicos dos que encontre en una busqueda ultra rapida}; b) a new model can be written. The main advantage of the first option is the effort savings (although you need to understand it) while its greatest disadvantage is that it might introduce a bias towards a particular verification environment/framework that you would not like to use. In turn the main advantage of the second choice is that you can use the tools that best suits your needs, but it has the disadvantage of taking longer to be ready. 
%
%In the present context we suggest to \hly{?????}.

For the present example we shall opt for the second alternative.% just because for a small example it could take a long time to learn a new semantics model. 
We specify just the elements we need for the present example. As specification language we use set theory and first-order logic.
We are thinking of providing two specifications: one using the Z language \cite{Spivey} and the other one using \texttt{Coq}.
%\hly{podriamos poner dos especificaciones una tipo Z y otra en Coq tratando de que las dos tengan mas o menos la misma semantica. yo hago la tipo Z. vean que les parece y si quieren meten la de Coq}

\verb+Transaction+ is a \verb+struct+. We will formalize this type as records. Then the semantics of \verb+Transaction+ is:
\begin{equation}
\begin{split}
Tran&saction \triangleq \\
[ & inputs:List(Input); \\
  & outpus:List(Output); \\
  & kernels:List(\mathit{TxKernel}); \\
  & \mathit{offset}: \mathit{BlindingFactor}]
\end{split}
\end{equation}
where, for instance, $List(Input)$ is the semantics assigned to \verb+Vec<Input>+ given that the latter is a {\it contiguous growable array type} (\url{https://doc.rust-lang.org/std/vec/struct.Vec.html}) %\hly{tener en cuenta que Vec parece ser algo en la stdlib de Rust y no algo primitivo} 
while the former is the type of lists\footnote{In set theory a list is an element of the set of partial functions, which in turn is a subset of the type of binary relations, which in turn is a synonym for the powerset of a given Cartesian product.}  of type $Input$.

Now \verb+PartialEq+ is function taking two arguments and returning a Boolean. In a first attempt we can model it as a binary relation, $\mathit{PartialEq}$, as follows:
\begin{equation}\label{partialeqdef}
\begin{split}
\texttt{PartialEq} & \texttt{(a,b) = true} \\
   & \iff (\llbracket a \rrbracket,\llbracket b \rrbracket) \in \mathit{PartialEq}
\end{split}
\end{equation}
where $\llbracket \cdot \rrbracket$ for any Rust construct means the semantics of that construct. In turn, $PartialEq$ can be defined as:
\begin{equation}
\begin{split}
\textit{Par}&\textit{tialEq} = \\
 & \{(x, y) \in Transaction \times Transaction \\
 &\quad\mid x.inputs = y.inputs \\
 &\qquad\land x.outputs = y.ouputs \\
 &\qquad\land x.kernels = y.kernels \\
 &\qquad\land x.\mathit{offset} = y.\mathit{offset}\}
\end{split}
\end{equation}

%\hly{aca medio que saque la guitarra (tal vez piensen que ya la habia sacado hace tiempo...) porque no conozco ni ahi la semantica de Rust y por lo que veo es mas compleja que lo que esta modelado. igual diria que como para dar una idea va. opinen.}

In this case both parameters are references to objects (of type \verb+Transaction+) in memory. Then, the semantics model should include a representation of objects in memory. We will model the memory as a partial function, $mem$, from memory addresses, $ADDR$, onto their contents. Besides we will model the notion embodied in the \verb+self+ construct by the $\mathit{self}$ variable. With these elements we can refine the predicate given in \eqref{partialeqdef} as follows:
\begin{equation}
\begin{split}
\texttt{Par} & \texttt{tialEq(\&self,tx:\&Transaction) = true} \\
   & \iff \mathit{self} \in Transaction \\
   &\hspace{9mm}\land mem(tx) \in Transaction \\
   &\hspace{9mm}\land (\mathit{self},mem(tx)) \in \mathit{PartialEq}
\end{split}
\end{equation}

%\hly{a continuacion se podria mostrar algunas de las pruebas o actividades de verificacion que se podrian hacer con este model. por ejemplo lo podria traducir a setlog y hacer alguna prueba medio boluda y alguna simulacion. que les parece?}

\hly{At this point we are inclined to illustrate the various possible uses of the model, showing how it can be translated to \{setlog\} and a simple proof can be carried out as well as some simulation of code execution.}

\subsection{Code verification}
\hly{TBC}



==> fm.tex <==
\section{Approaches to formal software verification}
\label{sec:afsv}

%In this section we comment on two general approaches to formal verification. 
Formal techniques can be applied in distinct phases of a software development project to different artifacts and aiming at different goals. Before choosing a formal technique to be applied it is necessary to define what artifacts need to be verified and the nature of the properties to be proved.

The universally accepted definition of program correctness is: \emph{a program is correct if it verifies its specification}. Usually, this specification is meant to be the \emph{functional specification} of the program. Given that in this work we are interested also in assessing the security of a software implementation we will take {\it program specification} as the functional and security specification of a program. Hence, in this context, \emph{a program is correct if it verifies its functional and security specifications}. 

We shall discuss in what follows two approaches to assess whether a program verifies its specification.

\subsection{From requirements to specification to code}
This is the classic approach proposed by the Software Engineering community when a brand new system is going to be developed. In this approach:
\begin{enumerate}
\item The development team writes down the \emph{requirements} of the system from the stakeholders' needs. The requirements of the system is typically a document written in natural language (sometimes accompanied by tables, illustrations, diagrams, etc.); i.e. it is an \emph{informal} description of the system. We will refer to this document as $R$.
%
\item From $R$ the development team elaborates a second document called software \emph{specification}. If a high degree of assurance of the final system is required this specification should be written using a \emph{formal notation}. We will refer to this document as $S$. Although formal, usually the specification is not executable, and if it does, it is usually very inefficient.
%
\item From $S$ the development team: a) elaborates a series of progressively more concrete specifications in such a way that the last document is an efficient program of $S$; or b) it directly writes a program. In any case, at least one new document is written: the program. We will refer to this document as $P$.
%
\item A number of \emph{verification activities} are carried out during the execution of the first three stages: 
%Just to name the most relevant to our context:
\begin{itemize}
\item Properties of $S$ are proposed, \emph{formalized} and \emph{proved}. In this sense, $S$ is taken as an axiomatic theory and theorems of this theory are proved. A typical class of properties of a much used class of specifications are \emph{state invariants}. The more theorems are proved the more confidence on the soundness and completeness of the theory (i.e., $S$) is gained. 

Failing to prove an expected property is a strong indication of some error in the specification. Usually these errors remain unnoticed until the final deployment of the system. Removing those errors as soon as possible usually implies significant cost reductions and avoid schedule overruns.
%
\item If a series of specifications ending in a program is written, $S_1,\dots,S_n,P$, each specification $S_{i+1}$ is proved to be an implementation (or a \emph{refinement}) of $S_i$, and $P$ is proved to be an implementation of $S_n$. This \emph{guarantees} or \emph{certifies} that $P$ is a correct implementation of $S$ (${}=S_1$).

If $P$ is written directly from $S$ then the above chain of transformation verifications is reduced to a single, usually more complex, proof.

In any case, a prerequisite for this activity is to have a \emph{formal} semantics of the implementation technology (essentially of the programming language).
%
\item Extensive testing is performed. %\hly{TBC}
\end{itemize}
\end{enumerate}


\subsection{\label{r2sc2s}From requirements to specification and from code to specification}
This approach can be seen as an adaptation of the first approach that can be used when at least a  substantial part of the system has already been implemented. Clearly, in this situation no formal $S$ is present (and in most cases no rigorous $R$ exists either) and, given that the there is an implementation, it is worthless to ask for a new implementation to be derived from the specification. Instead, the development team needs to check whether the existing implementation is correct or not, and in this last case to reveal all the errors. However, according to the definition of program correctness, checking the correctness of a given implementation can be done only w.r.t. a specification. Therefore, in this situation the following steps might be carried out:

\begin{enumerate}
\item\label{r} $R$ is written but usually from the existing project's documentation.
%
\item\label{s1} From $R$ a formal specification is generated; we will call it $S_1$.
%
\item\label{s1proof} Properties of $S_1$ are proved.
%
\item\label{s2} Another formal specification, called $S_2$, is derived from $P$. In this case, the structure (or design) of $P$ is considered. That is, each method, procedure, function, module, etc. in which $P$ has been divided or structured is formally specified. $S_2$ is the combination of the specification of all the elements of the design. Note that $S_2$ will predicate over the data structures and functions implemented by $P$, while $S_1$ will be more abstract.
%
\item\label{s2proof} Properties of $S_2$ are proved.
%
\item\label{s1s2} It is proved that $S_2$ is an implementation of $S_1$. If this proof fails, it should be analyzed whether the error is in $S_1$ or $S_2$. In general, $S_1$ should be considered more autoritative given that the correctness of the code is being assessed.
%
\item Extensive testing is performed. %\hly{TBC}
\end{enumerate}

Like in the previous approach, having a formal semantics of the implementation technology is a prerequisite. All steps from \ref{s2} to \ref{s1s2} can reveal errors in $P$. Steps \ref{r}-\ref{s1proof} can be executed at the same time than steps \ref{s2}-\ref{s2proof}, by two independent teams.


\subsection{Discussion}
As the main objective of this work is to provide certified guarantees of the correctness of an existing implementation of the protocol we propose to follow the second verification approach.
%For the present work we recommend to follow the second approach basically because there exist a working implementation of the protocol in question.
Therefore, $S_1$ and $S_2$ can be used to formalize issues or features that surface at two different levels of abstraction. For example, buffer overflows would be expressible only in $S_2$ because otherwise $S_1$ would be too concrete or detailed (note that buffer overflows depend strongly on the implementation technology; for instance, they are impossible in a Haskell program but they are common in C programs) so it makes no sense to mention them in $S_1$. On the other hand, the formalization of a property such as access control is easier to specify at the level of $S_1$ because abstract data structures (such as sets, binary relations or partial functions) can be used. Specifying the same property in $S_2$ would require to use implementation-level data structures such as singly-linked lists which would require to formalize references, dereferencing, pointer arithmetics, etc. That is, it would require to fill the specification with concepts that obscure its true goal: make it evident the access control property.

Different verification technologies enable or facilitate some of the activities mentioned above, while others will disable or complicate others. We would like to mention two examples:
\begin{itemize}
\item The proof-assistant \texttt{Coq} \cite{coq-manual} can automatically provide certified implementations. Indeed, under mild assumptions, after proving that some specification verifies a given property a computable version of that property can be automatically extracted from the proof. This implementation can be used as a prototype or as a first, bug-free, low-performance implementation.
%
\item Usually, formal specifications are not executable. However, state-based, set-based specifications can be easily (and most of the times automatically) translated into \setlog \cite{DBLP:conf/sefm/CristiaRF13}. This implies that, after writing a specification, a prototype is available for free. 
\end{itemize}


\subsection{Subtleties and traps with security properties}
In the present context, a formal definition of the security properties the system must verify is one of the most complex tasks. Security properties have proved to be unexpectedly complex to grasp and formalize. One of the fundamental reasons for this is that security properties are not safety properties (w.r.t. the Alper-Schneider framework). Most of the verification methods, results and tools developed for almost half a century by the Software Engineering community have been aimed at safety properties. Then, most of them fall short when dealing with security properties. Only very recently some of these methods and tools have been adapted for the problem of security properties.

For instance, safety properties enjoy, what is some times called, the \emph{refinement property}. This means that, if $S$ is the description of a system verifying safety property $F$ and $S'$ is a more deterministic refinement of $S$, then $S'$ (automatically) verifies $F$. However, in general, security properties do not enjoy the refinement property. This means that even if you have proved that $S$ verifies security property $F$ and that $S'$ is a refinement of $S$, then you cannot assert that $S'$ verifies $F$. The problem is that there are implementation decisions that in spite of generating a more deterministic system, they might introduce security issues. A typical example is the specification of the values stored in the memory cells delivered by the operating system to a process. At a certain level of abstraction these values might be underspecified which implies that, potentially, any value can be stored. Assume you can prove that this is secure. Afterwards, programmers decide to deliver the cells with the values left by the last process that used that buffer. Although this is an implementation of the first specification it is blatantly insecure.


On the other hand, reasoning about implementations provides the ultimate guarantee that
deployed mechanisms behave as expected. However, due to the issues mentioned above, formally proving non-trivial security properties of code might be an overwhelming task in terms
of the effort required, especially compared w.r.t. proving functional correctness (i.e. a safety property). In addition,
many implementation details are orthogonal to the security properties
to be established. This implies that slight changes in the implementation technology might have devastating consequences as concerns the security of the implementation. Therefore, complementary approaches are needed when non-trivial security properties are at stake:
\begin{enumerate}
\item Verification is performed on idealized models that abstract away the specifics of any particular implementation, and yet provide a realistic setting in which to explore the security issues that pertain to the realm of those (critical) mechanisms.
%
\item Additionally, verification is performed on more concrete models where low level mechanisms (such as pointer arithmetic) are specified. 
%
\item Finally, the low level model is proved to be a correct implementation of the idealized model.
\end{enumerate}

Note the similarities of this methodology w.r.t. the second approach outlined above.

%\subsubsection*{Security models}
%\emph{Security models} play an important role in the design and evaluation of high assurance security systems. Their importance was already pointed out in the Anderson report \cite{1296905}. The first model to appear was Bell-LaPadula \cite{Bell:LaPadula}, in 1973, in response to US Air Force concerns over the confidentiality of data in time-sharing mainframe systems.
%In the last decades, some countries developed specific security evaluation standards \cite{Criteria}. This initiative opened the path to worldwide mutual recognition of security evaluation results. In this direction, new Common Criteria (CC) \cite{Criteria2012}  was developed. CC defines seven levels of assurance for security systems (EAL 1--7). In order to obtain a higher assurance than EAL 4, developers require specification of a security model for security systems and verify security using formal methods. For example, the Gemalto and Trusted Logic companies obtained the highest level of certification (EAL 7) for their formalization of the security properties of the JavaCard platform \cite{coqjavacardeal7, formavie, Andronick:phd}, using the Coq proof assistant \cite{coqart,coq-manual}.

A particular class of the idealized models mentioned above are those called \emph{security models}. These models have played an important role in the design and evaluation of high assurance security systems. Their importance was already pointed out in the Anderson report~\cite{1296905}. The
paradigmatic Bell-LaPadula model~\cite{Bell:LaPadula}, conceived in 1973, constituted the first big effort on providing a formal setting in which to study and reason on confidentiality properties of data in time-sharing mainframe systems. 

\emph{State machines}, in turn, are a powerful tool that can be used for modeling many aspects of computing systems. In particular, they can be employed as the building block of
a security model. The basic features of a state machine model are the
concepts of state and state change. A \emph{state} is a representation
of the system under study at a given time, which should capture those
aspects of the system that are relevant to the analyzed problem. State
changes are modeled by a state transition function that defines the
next state based on the current state and input. If one wants to
analyze a specific safety property of a system using a state machine
model, one must first specify what it means for a state to satisfy the
property, and then check if all state transitions \emph{preserve} it.
Thus, state machines can be used to model the enforcement of a
security policy on a system.












==> prototype.tex <==
\section{Testing and monitoring in \texttt{Coq}}
\label{sec:prototype}
\newcommand{\exec}[4]{$#1 \overset{#2/#3}{\hookrightarrow} #4$}

% Certified security testing

%\hly{aca decidi encararlo un poco distinto. mas que nada pensando en que se supone que vamos a demostrar la correccion del codigo. en este caso el testing deberia cubrir los aspectos que un analisis estatico, como la prueba formal, no puede cubrir. por ejemplo uno puede haber axiomatizado cierta interfaz del sistema operativo o cualquier otro sistema externo que en la practica no verifica los axiomas. el testing podria/deberia descubrir esos problemas. que les parece? mas que nada trate de cambiar solo la introduccion o las partes mas coloquiales para ajustarlas al criterio anterior}

A system like the MimbleWimble protocol interacts with many other software systems. Some of these external systems are large and complex (e.g. the operating system and the TCP/IP protocol stack). When proving the correctness of a MimbleWimble implementation the interfaces of these external systems have to be axiomatized and thus assumed correct (because it would be impractical to prove the correctness of, say, the Linux operating system as a prerequisite to prove the correctness of MimbleWimble). However, these axioms might not describe the true behavior of these interfaces. Given that the proof of correctness of the MimbleWimble protocol depends on these axioms, if they are not accurate then MimbleWimble might behave unexpectedly. A similar analysis can be made when the compiler or runtime of the programming language on which MimbleWimble is implemented, is considered (i.e. they might not produce or execute code as assumed and a formal proof is out of scope). 

Since a formal proof is not feasible, extensive testing and monitoring may be the only tools to help in revealing many of these mismatches. Furthermore, this context is the ideal situation to apply: a) some model-based testing method; and b) a certified MimbleWimble's monitor. Both activities are based on using \texttt{Coq}'s program extraction mechanism. By using this \texttt{Coq}'s feature, we can derive a \emph{certified} Haskell prototype of the model described in Section \ref{sec:model}. This means that this Haskell program behaves exactly as described in the formal model and that it verifies \emph{all} of the security and functional properties that the model satisfies.

We briefly comment and motivate these two activities in what follows.


\subsection{\label{testing}Certified security testing}
%  because the formal model has already been developed for the formal proof
Model-based testing (MBT) is a lively research area whose main goal is to use
models of implementations as test case and oracle sources \cite{Utting00}. 
One of the possible high-level MBT processes is depicted in Figure \ref{f:mbt}. 
MBT methods based on such a process generate \emph{abstract test cases} by performing different
static analyzes of a (formal) model (of a given program). This abstract test
cases are later refined to the level of the program; the program
is run on these refined test cases; the outputs are collected and abstracted
away to the level of the model; and, finally, the model, the abstract test cases
and the abstracted outputs are used to decide whether the program has
errors or not. 

\begin{figure*}
\centering
\tikz [
    nonterminal/.style={
    rectangle, 
    minimum width=3.5cm, 
    minimum height=4mm,
    node distance=5mm,
    thick, 
    draw=black},
    >=Latex, arrows={[round]}] {
\node [nonterminal] (get) at (0,0) {get output};
\node [nonterminal] (abs) at (4.5,0) {abstract output};
\node [nonterminal] (vfys) at (9,0) {verify w.r.t. model};
\node [nonterminal] (set) at (9,1) {set initial values};
\node [nonterminal] (run) at (0,1) {run program};
%\node [nonterminal] (vfy) at (9,1) {verify output};
\node [nonterminal] (gen) at (1.42,2) {generate abstract test cases from model};
\node [nonterminal] (ref) at (9,2) {refine  test cases};
%\draw [dashed] (-2,0.5) rectangle (11,1.5);
\draw (gen) edge[->] (ref)
      (ref) edge[->] (set)
      (set) edge[->] (run)
%      (run) edge[->,dashed] (vfy)
      (get) edge[->] (abs)
      (abs) edge[->] (vfys)
      (run) edge[->] (get);
}
\caption{\label{f:mbt}Proposed MBT process}
\end{figure*}

In particular, for the generation of abstract test cases, a MBT method known as the Test Template Framework (TTF) \cite{Stocks2} can be applied. The TTF was originally thought as a MBT method for Z specifications \cite{Spivey:1989:ZNR:61690}  but it can be easily adapted to \texttt{Coq} models. 
In effect, a \texttt{Coq} model as the one we propose in Section \ref{sec:model} is a state machine featuring complex state and input variables and state transitions given by their pre- and post-conditions, much as Z specifications. Furthermore, pre- and post-conditions of our \texttt{Coq} axiomatic specification make use of non-trivial library operations on lists, similarly as Z specifications rest on library operations on sets. Besides, a tool such as \setlog has proved to be effective in abstract test case generation and in eliminating unfeasible test specifications.


\subsubsection*{The Test Template Framework} 
In the TTF the specification of the system under test (SUT) takes the form of a state machine (not necessarily a finite one). The TTF defines a methodology for generating abstract test cases for each state transition of the state machine. Then, let $A(\vec i,\vec s,\vec s',\vec o)$ be such an state transition depending on a vectors $\vec i$, $\vec s$, $\vec s'$, and $\vec o$ of, respectively, input, before-state, after-state and output variables\footnote{For the sake of simplicity, from now on, we will avoid the vector notation.}. Such an state transition is specified by its pre- and post-conditions: $A(i,s,s',o) \equiv Pre_A(i,s) \implies Post_A(i,s,s',o)$, where $Pre_A$ and $Post_A$ are two predicates.

The first step of the test case generation method of the TTF is to define the \emph{valid input space} of each state transition, which is the set of all possible values for $i$ and $s$ satisfying the precondition. Formally, $A^{VIS} \equiv \{(i,s) \mid Pre_A(i,s)\}$. 

As the second step, the TTF states that the VIS must be partitioned by a technique called \emph{recursive domain partition} (RDP). RDP is the core of the TTF. RDP starts by applying a \emph{testing tactic} to the VIS thus generating a partition of the VIS in the form of a collection of \emph{test specifications}. Each testing tactic describes how a test specification can be partitioned in order to obtain new and more demanding test specifications. A test specification is simply a set of test cases described by a predicate depending of the input and before-state variables. These predicates are called \emph{characteristic predicates}. Then, each testing tactic is defined by the collection of characteristic predicates that it generates. 

Hence, if testing tactic $T_a$ applied to $A^{VIS}$ generates the (characteristic) predicates $P^a_1,\dots,P^a_{n_a}$, the TTF states that $A$ has to be tested with test cases taken from the following test specifications:
\begin{gather*}
A^{T_a}_1 \equiv \{A^{VIS} \mid P^a_1(i,s)\} \\
A^{T_a}_2 \equiv \{A^{VIS} \mid P^a_2(i,s)\} \\
\dots \\
A^{T_a}_{n_a} \equiv \{A^{VIS} \mid P^a_{n_a}(i,s)\}
\end{gather*}

RDP continues by picking one or more of the $A^{T_a}_i$ and applying to them one or more testing tactics. For example, testing tactic $T_b$ can be applied to $A^{T_a}_2$ thus generating the following test specifications:
\begin{gather*}
A^{T_b}_1 \equiv \{A^{T_a}_2 \mid P^b_1(i,s)\} \\
A^{T_b}_2 \equiv \{A^{T_a}_2 \mid P^b_2(i,s)\} \\
\dots \\
A^{T_b}_{n_b} \equiv \{A^{T_a}_2 \mid P^b_{n_b}(i,s)\}
\end{gather*}

This process continues until engineers think they have a good coverage of the specification. The test specifications generated in this way can be accommodated in a so-called \emph{testing tree}. The testing tree has the VIS as its root node, the test specifications generated after applying the first testing tactic in the first level; the test specifications generated after applying more testing tactics to the first level, in the second level; and so forth. Note that the more testing tactics are applied, the more precise are the leaves of the testing tree. In effect, observe that the characteristic predicates of each testing tactic are conjoined to each other thus turning the characteristic predicates of leaves into conjunctions of several constraints. For example, if $A^{T_a}_2$ is expanded inside $A^{T_b}_2$ we have:
\begin{gather*}
A^{T_b}_2 \equiv \{A^{VIS} \mid P^a_2(i,s) \land P^b_2(i,s)\}
\end{gather*}

The third step in the TTF is to prune the unsatisfiable leaves off the testing tree. If the TTF is mechanically applied it tends to generate many unsatisfiable leaves as contradictory constraints can be conjoined in the same test specification. Depending on the theory used for the specification of the SUT, pruning can be an intractable problem but in general there exist algorithms that perform well in practice \cite{CristiaRossiSEFM13}.

The fourth and final step in the TTF is to generate an abstract test case from each surviving leaf of the testing tree. In this context, abstract test cases take the form of closed propositional sentences
binding state and input variables to concrete values. More precisely, an
abstract test case is a conjunction of equalities between variables and constant
terms. For example, if $A^{T_b}_3$ is a satisfiable test specification, its corresponding test case is described as follows:
\begin{gather*}
A^{TC}_3 \equiv \{A^{T_b}_3 \mid i = c_i \land s = c_s\}
\end{gather*}
where $c_i$ and $c_s$ are two constant (vector) terms. Observe that such a test case must verify all the characteristic predicates all the way up in the testing tree to the root node. Then, essentially, such a test case sets the initial state
and input values from which the state transition to be tested must be executed. In the TTF, test case generation is the dual problem of leaf pruning as both amount to solve the same satisfiability problem (i.e. determining whether test specifications are satisfiable or not) \cite{DBLP:journals/stvr/CristiaAFPM14}.

One of the advantages of the TTF is that it encourages that all the artifacts involved in the testing process (e.g. state transitions and test specifications) can be expressed in the same notation.
 
According to Figure \ref{f:mbt}, abstract test cases must refined into the implementation platform so they can be executed on the SUT. 
The final step in Figure 
 \ref{f:mbt} is to check whether each abstract output conforms with the corresponding abstract test case. 


\subsubsection*{Applying the TTF to \texttt{Coq} models}
The TTF can be easily applied to MimbleWimble's \texttt{Coq} specification. In particular the Haskell prototype derived from the specification can be used as the oracle engine given that it correctly implements the specification. However, some tools, \hly{like ...}, need to be developed for automating the MBT process described above. The development of those tools is technically feasible, the timing depends on the amount of resources invested.

%\hly{capaz que convendria mencionar que con el debido financiamiento esto se puede hacer mas o menos rapido}

\subsection{Monitoring MimbleWimble's implementation}
The testing process proposed in the previous section is meant to be applied \emph{before} the MimbleWimble implementation goes into production. Clearly, the idea of testing is a) to uncover errors in the implementation and b) that critical errors are fixed,  both before the system is delivered. However, as every one knows, testing will not always uncover all the errors. Hence, even after a formal proof of correctness and extensive testing, errors in or flawed assumptions about external systems may still be used to compromise the security of MimbleWimble.

For this last class of issues we propose to use the certified Haskell prototype. Indeed, this prototype can be used as the basis for a (on-line, quasi-real-time) monitor of MimbleWimble's implementation. In this setting:
\begin{enumerate}
\item MimbleWimble's implementation passes to the monitoring system every input it receives.
%
\item The monitor uses the abstraction harnessing mentioned in Section \ref{testing} to abstract the inputs it receives.
%
\item The Haskell prototype is called with the abstracted inputs, thus mimicking the execution of the implementation.
%
\item If the Haskell prototype transitions to an unexpected state an alarm is rose and, either automatically or after a human evaluation, the implementation can be stopped, suspended or some other protective measure can be taken.
\end{enumerate}

Clearly, the monitoring system will not be as efficient as the real implementation, what may cause some delay between the time MimbleWimble's implementation receives the offending input and the time the monitor raises an alarm. However, most likely, this input will be one in a rather long chain of interactions that eventually would end in compromising MimbleWimble. Therefore, in most of the cases the alarm rose by the monitoring system will help to avoid otherwise successful attacks or errors that may lead the system to disrupt critical data or functions.

Monitoring systems have been proposed for the enforcement of critical security properties \cite{DBLP:conf/csfw/ZanariniJR13}.



